Unveiling Project-Specific Bias in Neural Code Models

Deep learning has introduced significant improvements in many software analysis tasks. Although the Large Language Models (LLMs) based neural code models demonstrate commendable performance when trained and tested within the intra-project independent and identically distributed (IID) setting, they often struggle to generalize effectively to real-world inter-project out-of-distribution (OOD) data. In this work, we show that this phenomenon is caused by the heavy reliance on project-specific shortcuts for prediction instead of ground-truth evidence. We propose a Cond-Idf measurement to interpret this behavior, which quantifies the relatedness of a token with a label and its project-specificness. The strong correlation between model behavior and the proposed measurement indicates that without proper regularization, models tend to leverage spurious statistical cues for prediction. Equipped with these observations, we propose a novel bias mitigation mechanism that regularizes the model's learning behavior by leveraging latent logic relations among samples. Experimental results on two representative program analysis tasks indicate that our mitigation framework can improve both inter-project OOD generalization and adversarial robustness, while not sacrificing accuracy on intra-project IID data.

==> tex/IID.tex <==
\subsection{Why can BPR improve IID performance?}
From our experimental results, we observe that BPR also manages to improve performance on IID data beyond OOD generalization and adversarial robustness. We hypothesize that this is because during the early stage of the normal training process, the shortcut features have been rapidly picked up, which makes the model converge to local optima and hard to be updated by robust features. With the introduction of BPR, this \emph{shortcut convergence} process is inhibited and, therefore, more robust representations can be learned. We leave the detailed discussion to our future research.

==> tex/abstract.tex <==
\begin{abstract}
Deep learning has introduced significant improvements in many software analysis tasks. Although the Large Language Models (LLMs) based neural code models demonstrate commendable performance when trained and tested within the intra-project independent and identically distributed (IID) setting, they often struggle to generalize effectively to real-world inter-project out-of-distribution (OOD) data. In this work, we show that this phenomenon is caused by the heavy reliance on project-specific shortcuts for prediction instead of ground-truth evidence. We propose a Cond-Idf measurement to interpret this behavior, which quantifies the relatedness of a token with a label and its project-specificness. The strong correlation between model behavior and the proposed measurement indicates that without proper regularization, models tend to leverage spurious statistical cues for prediction. Equipped with these observations, we propose a novel bias mitigation mechanism that regularizes the model's learning behavior by leveraging latent logic relations among samples. Experimental results on two representative program analysis tasks indicate that 
our mitigation framework can improve both inter-project OOD generalization and adversarial robustness, while not sacrificing accuracy on intra-project IID data\footnote{Our code is available at \url{https://anonymous.4open.science/r/BPR_code_bias-F2AC/README.md}}.
\\ \newline \Keywords{keyword1, keyword2, keyword3} 
% as well as accuracy on IID data.

% To quantitatively evaluate such behavior, we propose a measure called cond-idf that combines co-occurrence probability and inverse document frequency to measure the level of relatedness of token with label and its project-specificness. We observe that the behavior of neural code models can be approximated with this metric, indicating that without proper injection of human knowledge, model prone to rely on tokens that are frequently co-occurred with the label yet are highly project-specific and hard to generalize. We further propose a general mitigation framework based on these observations, experimental results demonstrates that our framework can significantly increase model's performance on inter-project OOD setting. To the best of our knowledge, this is the first work that systematically studies the bias learning behavior of neural model for code representation learning.

% neural models strongly rely on the features that lies in the head of the ipf-LMI probability distribution, which are the tokens that frequently co-occur with the label yet are highly project-specific and hard to generalize. Besides, we further categorize these tokens into more fine-grained units with lexical analysis and observe that such tokens are gradually learned and their attention values increase monotonically throughout the training process. Based on the above two observations, we propose a novel framework to mitigate the project-specific shortcut learning behavior of code representation learning models.
\end{abstract}

==> tex/acknowledgement.tex <==
\section*{Acknowledgements}
This research is partially supported by the National Research Foundation, Singapore
 under its AI Singapore Programme (AISG Award No: AISG-PhD/2021-08-022[T]), the National Research Foundation, Singapore under its the
AI Singapore Programme (AISG2-RP-2020-019), the National Research Foundation, Prime Ministers
Office, Singapore under its National Cybersecurity R\&D Program (Award No. NRF2018NCR-NCR005-0001),
NRF Investigatorship NRF-NRFI06-2020-0001, the National Research Foundation through its National
Satellite of Excellence in Trustworthy Software Systems (NSOE-TSS) project under the National
Cybersecurity R\&D (NCR) Grant award no. NRF2018NCR-NSOE003-0001, the Ministry of Education,
Singapore under its Academic Research Fund Tier 1 (21-SIS-SMU-033), Tier 2 (MOE2019-T2-1-040) and
Tier 3 (MOET32020-0004). Any opinions, findings and conclusions or recommendations expressed in
this material are those of the author(s) and do not reflect the views of the Ministry of Education,
Singapore.

==> tex/append-baseline.tex <==
\subsection{Baseline details}
\begin{itemize}[leftmargin=*]
  \item \textbf{Reweighting}: 
  This method first trains a bias-only model using recognized bias. Empirically, the bias-only model is often confident about its prediction and assigns high probability to samples with bias. Given with the confidence predicted by the bias-only model $p_{b}^{i}$, to train a de-biaed model, the classification loss of each training loss is reweighted with $1-p_{b}^{i}$ so that samples that exhibit bias are expected to be downweighted. Formally:
  \begin{equation}
      \mathcal{L}_\mathrm{DEBIAS}=-\mathbb{E}_{(x_i, x_j) \sim D}\left(1-p_{b}^{i}\right) y^{i} \cdot \log p_{d}^{i}
  \end{equation}
  where $p_{d}$ is the normalized predicted probability distribution of the debiased model. Specifically, in our implementation, for vulnerability detection, the bias-only model is trained on user-define variable and function names as well as macro-definitions; for type inference, the bias-only model is trained merely on the declaration variable representation. We use the CodeBert architecture for the bias-only model, which is the same as the debiased model.
  \item \textbf{Product-of-expert (PoE)}: Similarly to re-weighting, PoE also requires a trained bias-only model. The debiased model is trained in an ensemble manner with the bias-only model by combining their normalized prediction probability, which is as follows:
  \begin{equation}
      \mathcal{L}_\mathrm{DEBIAS}=-\mathbb{E}_{(x_i, y_i) \sim D}y^{i} \cdot \log \operatorname{softmax}[\log (p_{d}^{i} \cdot p_{b}^{i})]
  \end{equation}
  For PoE, the biased models we used are the same as those used in reweighting.
  
  \item \textbf{Adversarial training}: 
  Instead of updating the model with only original samples, adversarial training\cite{madry2017towards,goodfellow2014explaining} proposes to train the model with perturbed adversarial samples along with the original ones so that the model is expected to perform robustly when handling data with perturbations. Formally:
  \begin{equation}
      \mathcal{L}_\mathrm{DEBIAS}=-\mathbb{E}_{(x_i, x_i', y_i) \sim D} \mathcal{L}(x_i, y_i) + \mathcal{L}(x_i', y_i)
  \end{equation}
  where $x_{i}'$ is a perturbed version of the original sample $x$. In our implementation, we follow Yefet~\etal\cite{yefet2020adversarial} to perturb samples with non-targeted attack using single BFS step on the recognized bias tokens.
  
  \item \textbf{Gradient Reversal}:
  The methods propose to unlearn bias information explicitly in a minimax game manner. Specifically, it employs an additional bias prediction network $h$ to predict the bias distribution along with the standard target classification loss and update the weights of the backbone model adversarially by reversing the gradient of the bias prediction network so that at the end of training, the bias prediction network is unable to predict bias, since the backbone model $f$ has successfully unlearned the bias. Formally:
  \begin{equation}
  \begin{aligned}
      \min _{\theta_{f}, \theta_{g}} \max _{\theta_{h}}&\mathbb{E}_{(x_i, y_i) \sim D} \mathcal{L}(x_i, y_i;\theta_{f}, \theta_{g}) \\ &- \mu\mathcal{L}(b(x_i), h\circ f(x_i; \theta_{f},\theta_{h}))
  \end{aligned}
  \end{equation}
  where $g$ is the classification head layer for the regular target classification, $b(x_i)$ is the known bias of a sample $x_i$, in our case, it is the bias vocabulary set, $\mu$ is a regulatory coefficient which is set as 0.1 in our implementation.
  
\end{itemize}

==> tex/append-case.tex <==
\subsection{More Case Studies}
We present more case studies to analyze the effectiveness of BPR. For vulnerability detection, we show a memory leak vulnerability in Figure~\ref{case_study2}, whose commit ID is \textbf{cdf3606b384b434fbadae0751f9b4024de8bf177}. Specifically, this vulnerability is caused by \emph{Dangling Pointer}, if the memory that struct \emph{g} refers to is freed: \emph{free(g-\textgreater sarea);free(g);} , pointer \emph{ap} would potentially form a \emph{Dangling Pointer}: \emph{ap = g-\textgreater activitystart;}, and causes memory leak vulnerability. Therefore, in order to infer such case as vulnerable, model should focus on the above-mentioned statement. The visualization of the attribution vector indicates that the original model infers on the basis of spurious bias and completely ignores the ground-truth evidence. After debiasing with gradient reversal, though the model starts to pay attention to ground-truth evidence, it biases on a new function name subword \emph{xit} and falls to predict correctly. Finally, by combining BPR, the model attributes much higher weights to the ground truth evidence that is used to infer \emph{Dangling Pointer} and predicts correctly. Figure~\ref{case_study3} shows the visualization of a type infer example. In order to predict the type of variable \emph{\_i} as number, model should and only should focus on the assignment \emph{var \_i = 0;}. It is obvious that the original model fails to leverage the ground-truth evidence. Though adversarial training manages to force model to use the ground-truth evidence, it still heavily biases on irrelevant tokens and infers erroneously. With the introduction of BPR, model makes correct inferences based on ground-truth evidence.


